VibeVideoBench: Evaluating Multimodal Agents on Code-Driven Video Generation

Multimodal agents can create videos by writing code and coordinating rendering and audio tools. Yet it remains unclear how reliably they can turn detailed specifications into complete videos. We introduce VibeVideoBench, a benchmark of 239 self-contained tasks across 12 categories in English and Chinese. Agents operate in their native harnesses within a sandbox and must deliver a finished video within one hour, with audio as required. No image or video generation models are available. Evaluation combines programmatic delivery checks, approximately 13,000 task-specific rubric checks, and whole-video quality assessment. Across nine frontier agent systems and 2,151 rollouts, GPT-6 Astra and Claude Opus 5.5 lead both the judge-based quality ranking and the human preference ranking. However, the highest strict task-success rate is only 76.3%. Agents typically build custom rendering pipelines, but their outputs still exhibit errors in required actions, state changes, and timing. Execution traces also reveal gaps between identifying a defect, revising the code, and delivering a corrected video. VibeVideoBench provides a testbed for evaluating video production as an end-to-end agent task, encompassing requirement satisfaction, audiovisual quality, and delivery reliability.

==> tables/main_rows.tex <==
\vvbmodel{openai}{GPT-6 Astra} & Codex CLI & 238 & 93.7 & 97.1 & \vvbbest{vvbscorewash}{4.126}{0.825211} & \textbf{1242} & 74.5 & \vvbbest{vvbzerowash}{4.109}{0.821727}\,{\scriptsize\textcolor{black!45}{(1)}} \\
\vvbmodel{claude}{Claude Opus 5.5} & Claude Code & \textbf{239} & \textbf{99.6} & \textbf{97.3} & \vvbbar{vvbscorewash}{4.074}{0.814893} & 1203 & \textbf{76.3} & \vvbbar{vvbzerowash}{4.074}{0.814893}\,{\scriptsize\textcolor{black!45}{(2)}} \\
\vvbmodel{claude}{Claude Sonnet 5.5} & Claude Code & 232 & 94.6 & 93.9 & \vvbbar{vvbscorewash}{3.999}{0.799804} & 1121 & 67.0 & \vvbbar{vvbzerowash}{3.880}{0.776021}\,{\scriptsize\textcolor{black!45}{(4)}} \\
\vvbmodel{gemini}{Gemini 4 Argon} & Antigravity CLI & 184 & 76.6 & 96.5 & \vvbbar{vvbscorewash}{3.989}{0.797737} & 1081 & 55.2 & \vvbbar{vvbzerowash}{3.069}{0.613720}\,{\scriptsize\textcolor{black!45}{(7)}} \\
\vvbmodel{deepseek}{DeepSeek-V4.1-Flash} & DSH & 236 & 94.6 & 93.1 & \vvbbar{vvbscorewash}{3.961}{0.792182} & 1022 & 57.6 & \vvbbar{vvbzerowash}{3.911}{0.782158}\,{\scriptsize\textcolor{black!45}{(3)}} \\
\vvbmodel{kimi}{Kimi K3} & Kimi Code & 213 & 85.8 & 91.1 & \vvbbar{vvbscorewash}{3.864}{0.772780} & 997 & 46.3 & \vvbbar{vvbzerowash}{3.440}{0.688066}\,{\scriptsize\textcolor{black!45}{(5)}} \\
\vvbmodel{zai}{GLM-5.3-Flash} & ZCode & 179 & 66.9 & 85.3 & \vvbbar{vvbscorewash}{3.736}{0.747248} & 905 & 33.5 & \vvbbar{vvbzerowash}{2.790}{0.557934}\,{\scriptsize\textcolor{black!45}{(9)}} \\
\vvbmodel{openai}{GPT-5.6 Sol} & Codex CLI & 213 & 84.5 & 89.5 & \vvbbar{vvbscorewash}{3.735}{0.746935} & 705 & 39.0 & \vvbbar{vvbzerowash}{3.317}{0.663329}\,{\scriptsize\textcolor{black!45}{(6)}} \\
\vvbmodel{gemini}{Gemini 3.8 Flash} & Antigravity CLI & 193 & 77.4 & 80.5 & \vvbbar{vvbscorewash}{3.470}{0.694089} & 723 & 26.6 & \vvbbar{vvbzerowash}{2.798}{0.559621}\,{\scriptsize\textcolor{black!45}{(8)}} \\


